Critical Drift for Brownian Bees and a Reflected Brownian Motion Invariance Principle

$N$-Brownian bees is a branching-selection particle system in $\mathbb{R}^d$ in which $N$ particles behave as independent binary branching Brownian motions, and where at each branching event, we remove the particle furthest from the origin. We study a variant in which $d=1$ and particles have an additional drift $\mu\in\mathbb{R}$. We show that there is a critical value, $\mu_c^N$, and three distinct regimes (sub-critical, critical, and super-critical) and we describe the behaviour of the system in each case. In the sub-critical regime, the system is positive Harris recurrent and has an invariant distribution; in the super-critical regime, the system is transient; and in the critical case, after rescaling, the system behaves like a single reflected Brownian motion. We also show that the critical drift $\mu_c^N$ is in fact the speed of the well-studied $N$-BBM process, and give a rigorous proof for the speed of $N$-BBM, which was missing in the literature.

==> sections/discuss.tex <==
As we noted in the introduction the behaviour of the $N$-Brownian bees system without drift is known when the number of particles tends to $\infty$. In particular, it is known that as $N\to\infty$, the empirical distribution of particles converges to the solution of a free boundary problem given by:
\begin{align} \label{beesFBP1}
\begin{cases}
    u_t=\frac{1}{2}u_{xx} + u  & x\in(-R_t,R_t), t>0, \\
    \int_{-R_t}^{R_t} u(s,t)ds=1 & t>0, \\
    u(t,x)=0 &  x\notin (R_t,R_t), t>0,
\end{cases}
\end{align}
with an initial condition based on the initial distribution of particles. This result is proven by Berestycki et al. in \cite{afree}, \cite{beesBBNP}.

We conjecture that for Brownian bees with sub-critical drift $\mu$ such that $|\mu|<\mu_c^N$, the empirical distribution converges to the solution of the FBP:
\begin{align}
\begin{cases}
    u_t=\frac{1}{2}u_{xx} - \mu u_x + u  & x\in(-R_t,R_t), t>0, \\
    \int_{-R_t}^{R_t} u(s,t)ds=1 & t>0, \\
    u(t,x)=0 &  x\notin (R_t,R_t), t>0.
\end{cases}
\end{align}

The methods of proof used by Berestycki et al. rely on the symmetry of the system, and view it essentially as a system of reflected Brownian motions on $[0,\infty)$. However these methods no longer work when drift is introduced, since $|B_t + \mu t|$ does not behave like a reflected Brownian motion and in fact is not even Markovian. Therefore this conjecture remains open.


